A Systematic Survey on Debugging Techniques for Machine Learning Systems

Debugging ML software (i.e., the detection, localization and fixing of faults) poses unique challenges compared to traditional software largely due to the probabilistic nature and heterogeneity of its development process. Various methods have been proposed for testing, diagnosing, and repairing ML systems. However, the big picture informing important research directions that really address the dire needs of developers is yet to unfold, leaving several key questions unaddressed: (1) What faults have been targeted in the ML debugging research that fulfill developers needs in practice? (2) How are these faults addressed? (3) What are the challenges in addressing the yet untargeted faults? In this paper, we conduct a systematic study of debugging techniques for machine learning systems. We first collect technical papers focusing on debugging components in machine learning software. We then map these papers to a taxonomy of faults to assess the current state of fault resolution identified in existing literature. Subsequently, we analyze which techniques are used to address specific faults based on the collected papers. This results in a comprehensive taxonomy that aligns faults with their corresponding debugging methods. Finally, we examine previously released transcripts of interviewing developers to identify the challenges in resolving unfixed faults. Our analysis reveals that only 48 percent of the identified ML debugging challenges have been explicitly addressed by researchers, while 46.9 percent remain unresolved or unmentioned. In real world applications, we found that 52.6 percent of issues reported on GitHub and 70.3% of problems discussed in interviews are still unaddressed by research in ML debugging. The study identifies 13 primary challenges in ML debugging, highlighting a significant gap between the identification of ML debugging issues and their resolution in practice.

==> OldRQ3.tex <==
\subsection{RQ3: Which faults have been targeted by ML debugging techniques, but are not included in the existing taxonomy of faults?}\label{subsec:targetednomentioned}
\bachle{Need to cite ML debugging papers that targeted each category of these faults.}
To understand how targeted faults are being addressed, we constructed a taxonomy of debugging techniques based on the collected literature as we described in detailed in Section~\ref{subsec:taxonomydebugging}. This results in the lower part of Figure~\ref{fig:taxonomy_of_alignment}. Overall, the taxonomy consists of 8 themes: \textit{Trained Models Fix}, \textit{Hyper Parameter Repair}, \textit{Defect Diagnostic}, \textit{Testing}, \textit{Attribution-based Detection of Data And Model Incompatibility}, \textit{Low-quality data debugging}, \textit{Active-learning-based Training Data Re-labeling} and \textit{API Fuzzing}. The taxonomy also consists of arrows connecting the taxonomy of faults to the corresponding fixing techniques that can fix them.
We describe in detail these techniques and how they address the corresponding faults below.

\noindent\textbf{Trained Model Fix.} The trained model fix consists of a total of 12 papers. It consists of 5 subcategories: Ensembling models~\cite{Chen2022MAAT}, Weight Update, Code Refactoring for Performance Optimization, and Similarity-based Model Prediction Correction. All of these techniques are used to address \textbf{Trained Weights} from the model category, which is an unmentioned problem. \textit{Ensembling models}~\cite{Chen2022MAAT} combines the model trained with different objectives for improving the fairness and performance bugs of deep learning models. \textit{Weight Update} updates the weights of model either by weights search~\cite{Sun2022Care} or retraining by adding additional samples~\cite{deepmetis}. \bachle{Citation missing. Also other things such as Code Refactoring, etc are missing/not explained yet.}

\bachle{C+E, or C+E+G}
\bachle{We should cite papers that address each categories and explain how they do it briefly. Perhaps, we already did cite them here, but the way we cite/explain wasn't yet very obvious}

\noindent\textbf{API Error}  Although the development of machine learning algorithms may involve automated processes and data-driven decision-making, the platforms and systems that implement these algorithms are firmly rooted in human-designed frameworks. Such structures, including APIs, are susceptible to the same types of errors and oversights commonly found in traditional software development~\cite{pham2019cradle}.
Therefore, established principles employed in detecting and rectifying faults in conventional software systems are still highly relevant when identifying issues in machine learning implementations.
The most prominent direction is revealing these faults through testing, either via fuzzing, metamorphic testing or differential testing between different APIs~\cite{pham2019cradle}.

\noindent\textbf{Model Fairness} In machine learning, model fairness refers to the objective of ensuring that predictive models do not produce biased outcomes that disproportionately affect certain groups, particularly those defined by sensitive attributes like race, gender, or socioeconomic status. An unfair model, even if it performs well in terms of accuracy, may unintentionally discriminate against specific subgroups by making biased predictions, leading to negative societal consequences such as biased hiring, unequal loan access, or discriminatory law enforcement decisions \cite{hardt2016equality, barocas2017fairness, zliobaite2017fairness}.



\noindent\textbf{Low-quality test set} Both traditional software systems and machine learning models, despite their contrasting building methodologies, share a common dependency: the quality of their test sets. For traditional software, well-constructed test cases ensure functional correctness and performance optimization. In the context of machine learning, a quality test set ensures that the model can generalize well to unseen data. If test sets contain duplications, data leakage, or fail to cover all behaviors of the neural networks, they risk becoming ineffective and misleading during evaluation. A poor-quality test set in machine learning might allow a model to achieve deceptively high accuracy by inadvertently including training data or highly similar data points, which leads to data leakage, ultimately reducing the real-world applicability of the model \cite{Humbatova2020taxonomyofrealfault,pham2019cradle}. Furthermore, inadequate test sets may fail to capture edge cases or adversarial inputs, resulting in overfitting to the test data and an inability to generalize to novel, challenging inputs \cite{pei2017deepxplore,ma2018deepgauge}. This lack of diversity and representativeness in the test set can cause the machine learning model to perform well under controlled conditions but fail in production environments, where data distributions and behaviors differ from those seen during training and testing. As a result, ensuring high-quality, diverse, and representative test sets is crucial to avoiding hidden defects in both traditional software and machine learning models.

\noindent\textbf{Data and Model Incompatibility} Data and model incompatibility is a common type of fault in machine learning systems that arises when the characteristics of the input data do not align with the expected format or structure of the machine learning model. This type of fault can manifest in several ways, including mismatched data types, incorrect input dimensions, or invalid feature representations, leading to suboptimal or erroneous predictions.
Detecting and addressing data-model incompatibility is crucial for ensuring that machine-learning models function correctly and continue to perform well as the input data evolves.
